Enhancing Consistency-Based Image Generation via Adversarialy-Trained Classification and Energy-Based Discrimination

The recently introduced Consistency models pose an efficient alternative to diffusion algorithms, enabling rapid and good quality image synthesis. These methods overcome the slowness of diffusion models by directly mapping noise to data, while maintaining a (relatively) simpler training. Consistency models enable a fast one- or few-step generation, but they typically fall somewhat short in sample quality when compared to their diffusion origins. In this work we propose a novel and highly effective technique for post-processing Consistency-based generated images, enhancing their perceptual quality. Our approach utilizes a joint classifier-discriminator model, in which both portions are trained adversarially. While the classifier aims to grade an image based on its assignment to a designated class, the discriminator portion of the very same network leverages the softmax values to assess the proximity of the input image to the targeted data manifold, thereby serving as an Energy-based Model. By employing example-specific projected gradient iterations under the guidance of this joint machine, we refine synthesized images and achieve an improved FID scores on the ImageNet 64x64 dataset for both Consistency-Training and Consistency-Distillation techniques.

==> Sections/method.tex <==
\section{Proposed Approach - Roy}
We propose a method for refining the perceptual quality of consistency models-based generated images as a post-processing step.
To this end, we train a joint classifier-discriminator-based network to guide the synthesized images toward better ones via pixel-space optimization.
We propose a method for post-processing Consistency-based generated images, enhancing their perceptual quality. Our approach utilizes a joint classifier-discriminator, in which both portions are trained adversarially. 
the model leverages the classifier's logits directly to perform as a discriminator within the same architecture. The distinction lies in how these logits are interpreted and utilized differently for the discriminator's task, as opposed to the straightforward classification task. In this case, the discriminator leverages the softmax values to assess the proximity of the input image to the targeted data manifold, thereby serving as an Energy-based Model.

Our methodology draws significant inspiration from BIGROC. Robust classifiers trained through adversarial methods are less susceptible to adversarial attacks and tend to produce gradients that are more aligned with human visual perception. This leads to enhancements in the image that are meaningful and visually coherent, rather than arbitrary pixel modifications. Although these improvements are significant, they lack an understanding of the real data distribution and therefore cannot distinguish between real and fake images. Our approach extends this by incorporating a discriminator within the same architecture. This discriminator evaluates how close the images are to the actual data distribution. The core concept is to train our classifier by exposing it to both the distribution of real data, $p_{real}$, and the distribution of synthesized data, $p_{generated}$, as opposed to the conventional approach of training robust classifiers solely with $p_{real}$. This dual exposure allows the classifier to better distinguish between real and synthetic images by understanding the characteristics unique to each distribution. This approach enhances the classifier's ability to accurately identify and enhance the realism of generated images while maintaining their intended characteristics.

While the concept of Energy-Based Models (EBMs) aligns perfectly with our task to improve image generation quality, they come with several challenges that impact their practical application. First, EBMs often require careful tuning of their learning parameters, as the energy landscape they model can be complex and difficult to navigate. This complexity can lead to issues with training stability, where the model may fail to converge or converge to undesirable local minima, resulting in poor generalization of new data. Additionally, EBMs are sensitive to the choice of the energy function. An inadequately defined energy function can lead to a model that either assigns high probability to non-data-like samples or fails to capture the diversity of the dataset, thereby affecting the quality of the generated images.
The training objective usually used in EBMs aims to adjust $p_\theta(x)$ given in equation \eqref{3} such that the model's energy surface aligns with the data distribution, the loss function often employed is based on minimizing the difference between the energy of the real data and the expected energy of the model distribution. The objective is typically formulated as:
\begin{equation}\label{6}
\mathcal{L}(\theta) = \mathbb{E}_{x\sim p_{data}}[E_\theta(x)] - \mathbb{E}_{x\sim p_{\theta}}[E_\theta(x)]
\end{equation}
Where $E_\theta$ is the energy function and $\theta$ is the model parameters. This expression is often approximated using sampling techniques like Markov Chain Monte Carlo (MCMC) because directly computing expectations under $p_\theta$ is computationally infeasible due to the unknown partition function $Z(\theta)$.

EBMs require extensive computational resources, particularly due to the need for sampling during training. Sampling methods such as Markov Chain Monte Carlo (MCMC) are computationally expensive and slow, especially when dealing with high-dimensional data like images and the ImageNet dataset in particular. The complexity and variety within ImageNet demand a model that can capture a vast range of features and variations, pushing the limits of an EBM’s capacity to model such diverse data effectively.

Given the challenges previously discussed, we propose a revised interpretation of the training objective. The classifier is employed to differentiate between samples from $p_{real}$ and $p_{gen}$ using the following equation:

\begin{equation}\label{7}
\mathcal{L}(\theta) = \mathbb{E}_{x\sim p_{data}}[log f_\theta^c(\hat{x})] + \mathbb{E}_{x\sim p_{\theta}}[log(1-f_\theta^c(\hat{x}))]
\end{equation}

In this formula, $\hat{x}$ represents the adversarially attacked example of $x$, $f_\theta$ is a classifier and $c$ is the class to which sample $x$ belongs. The above is closely related to GAN's training objective, but can also be interpreted as an energy-based training. 
Both the EBM loss function and the proposed training objective aim to minimize the energy (or increase the likelihood) of observed data points and maximize the energy (or decrease the likelihood) of sampled/generated data points. In EBMs, this is done by reducing the energy of real data samples and increasing it for generated samples. In the logistic regression-based approach, the likelihood of the real data under the model (represented by $f_\theta^c(x)$) is maximized, while the likelihood of the generated data (represented by $(1-f_\theta^c(x)$) is minimized.

\subsection{Training a Joint Classifier-Discriminator} 
Inspired by the discussion above, we propose the following loss function:

\begin{equation}\label{8}
\mathcal{L} = \mathcal{L}_{CE}(\hat{x}_{real}) + \mathcal{L}_{CE}(\hat{x}_{gen}) + \mathcal{L}_{BCE}(\hat{x}_{real}) + \mathcal{L}_{BCE}(\hat{x}_{gen})
\end{equation}

The proposed loss function integrates multiple components, each targeting specific aspects of the training.
The Cross-Entropy loss on perturbed real samples $\hat{x}_{real}$, ensures that the classifier can accurately classify real images to their correct classes despite any potential adversarial modifications, thereby reinforcing the model's resilience to adversarial attacks and maintaining high classification accuracy on real data.
Similarly, this term calculates the CE loss for the generated image, maintaining the model's ability to classify generated images correctly into a designated 'fake' class.
This encourages the model to recognize and categorize synthetic data accurately, which is crucial for distinguishing between real and fake images effectively.
The Binary-Cross-Entropy loss is:

\begin{equation}\label{9}
\mathcal{L}_{BCE}(z_c, t) = - t \cdot log(z_c) - (1-t) \cdot log(1-z_c)
\end{equation}

Where $t$ is a binary indicator where  $t=1$ if $\hat{x}$ is a real images and 0 otherwise, the output $z_c = f_\theta^c(\hat{x})$ is the probability assigned by the classifier that $\hat{x}$ belongs to class $c$.
For real images, the loss simplifies to:
\begin{equation}\label{10}
\mathcal{L}_{BCE}(z_c, 1) = -log(z_c)
\end{equation}
Which penalizes the model if it assigns a low probability to a real image.
And for fake images, 
\begin{equation}\label{11}
\mathcal{L}_{BCE}(z_c, 0) = -log(1-z_c)
\end{equation}
The model is penalized for assigning high probability values to a fake image.

This loss formulation ensures that the classifier learns to distinguish effectively between the two categories, enhancing its ability to deal with adversarially altered images and to generalize well across different types of image manipulations.

Our adversarial examples are generated using PGD (Projected Gradient Descent) attacks, as described in Algorithm 1. PGD uses a deterministic approach to gradient ascent, meaning it follows a predefined path based on the gradient of the loss function with respect to the input. This method, while robust, tends to explore only a limited area around the starting point of each input sample.
Therefore, its effectiveness in exploring diverse local maxima is inherently tied to the variety present in the initial samples. To mitigate this limitation, we propose a strategy of gradually increasing the number of attack steps throughout the training process. By extending the number of steps, the PGD attack can move further from the initial starting points, exploring new and potentially more challenging adversarial examples. Moreover, as the model becomes more adept at countering simpler attacks, incrementally increasing the complexity of the attack ensures that the training continues to challenge the model effectively.
To ensure the model does not mistakenly classify high-quality but still fake samples as genuine, we implement an early stopping mechanism based on the model's probability outputs. This mechanism halts the Projected Gradient Descent (PGD) process when the model assigns a higher probability to a perturbed fake image being real than it does to a perturbed real image. If such a situation occurs, we will not take further PGD steps in that direction.
This mechanism prevents the model from being misled by sophisticated fake samples that closely mimic real images. It ensures that the model's training does not reinforce incorrect classifications, which could degrade its performance in practical scenarios. By stopping further adversarial modifications when the model begins to confuse fake for real images, we preserve the reliability and discriminative power of the model against varying levels of adversarial attacks.

\subsection{Boosting Process} 

\begin{algorithm}
\caption{}\label{alg:cap}
\begin{algorithmic}
\State \textbf{Input:} 

Robust Classifier $f_\theta(x)$,

Input image x, and 

Algorithm's parameters: Radius $\varepsilon$, 
Step-size $\alpha$, No. of iterations $T$, 

$p_{real}$ threshold.

\State Set $\delta_0 \gets 0$.
\State Set ${\hat c} = f_\theta(x)$.
\For{$t$ from $0$ to $T$}
   \State $\delta_{t+1} = \Pi_\varepsilon(\delta_t-\alpha\nabla_\delta \left(\mathcal{L}_{CE}(f_\theta(x+\delta_t),{\hat c}) \right) - \frac{1}{2} (\mathcal{L}_{BCE}(f_\theta(x+\delta_t),{0})-p_{real})^2))$.
\EndFor
\State \textbf{Output:} $x_{adv} \gets x+\delta_T$
\end{algorithmic}
\end{algorithm}
